A Faster Algorithm for Quickest Transshipments via an Extended Discrete Newton Method

The Quickest Transshipment Problem is to route flow as quickly as possible from sources with supplies to sinks with demands in a network with capacities and transit times on the arcs. It is of fundamental importance for numerous applications in areas such as logistics, production, traffic, evacuation, and finance. More than 25 years ago, Hoppe and Tardos presented the first (strongly) polynomial-time algorithm for this problem. Their approach, as well as subsequently derived algorithms with strongly polynomial running time, are hardly practical as they rely on parametric submodular function minimization via Megiddo's method of parametric search. The main contribution of this paper is a considerably faster algorithm for the Quickest Transshipment Problem that instead employs a subtle extension of the Discrete Newton Method. This improves the previously best known running time of $\tilde{O}(m^4k^{14})$ to $\tilde O(m^2k^5+m^3k^3+m^3n)$, where $n$ is the number of nodes, $m$ the number of arcs, and $k$ the number of sources and sinks.

==> 4_Integral.tex <==
The quickest transshipments we compute in the previous section are fractional in the sense that we allow fractional flow values, that change at fractional times. Since the optimal time horizon can be fractional, it is clear that flow value changes at fractional times are necessary for quickest transshipments. Thus, given integral supplies, demands, and capacities, the goal of this section is to compute \textit{Integral Quickest Transshipments}, which are Quickest Transshipments with integral flow values.

HoTa only allow an integral time horizon with integral flow values, that change at integral times. This is the discrete time model...???\todo{right?}

Inspired by HoTa...


\begin{algorithm}[h]
	\DontPrintSemicolon
	\caption{Integral Quickest Transshipments}
	\label{Alg:integral}
	\KwIn{a dynamic network $\N$ and a supply/demand vector $b$ with integral supplies, demands, and capacities}
	\KwOut{minimal feasible time horizon $\theta^*$ and an integral Quickest Transshipment for $(\N,b)$}
	
	Use Algorithm~\ref{alg_main} to compute the minimal feasible time horizon $\theta^*$\;
	Initialize the chain $\mathcal C=\{\emptyset,S^+\cup S^-\}$\;
	\While{there are adjacent $Q\subsetneq R \in\mathcal C$ with $|R\backslash Q|>1$}{
		Choose $s_i\in R\backslash Q$ connected to $s$ {\color{red} $s_i$ still ``free'' after uncrossing?}\;
		\If {$Q+s_i$ is tight} { add $Q+s_i$ to $\mathcal C$ and \textbf{continue}}
		Use Algorithm~\ref{Alg:param_transit} to find a $\gamma$ s.t. $(\mathcal N_{\mathcal C,s_i}^\gamma,v_{\mathcal C,s_i}^\gamma,\theta^*)$ is feasible but $(\mathcal N_{\mathcal C,s_i}^{\gamma+\varepsilon},v_{\mathcal C,s_i}^{\gamma+\varepsilon},\theta^*)$ is infeasible\;
		Determine a violated set $T$ in $(\mathcal N_{\mathcal C,s_i}^{\gamma+\varepsilon},v_{\mathcal C,s_i}^{\gamma+\varepsilon},\theta^*)$ via a submodular function minimization\;
		Add $T$ and $R+s_{i+1}$ to $\mathcal C$\; 
		Add $s_i$ to all $R\subsetneq U\in\mathcal C$\;
		Add $s_{i+1}$ to $\N$\;
		Uncross $\mathcal C$\;
	}
	\Return \textsc{Lex-Max-Flow}$(\mathcal C)$
\end{algorithm}

\begin{theorem}
Algorithm~\ref{Alg:integral} returns an integral solution to a Quickest Transshipment Problem with integral supplies, demands, and capacities.
\end{theorem}
\begin{proof}
Inspired by HoTa...

write out the uncrossing chain...
\end{proof}

\begin{lemma}
Algorithm~\ref{Alg:integral} terminates within $O(k)$ iterations.
\end{lemma}

Def $(\mathcal N_{\mathcal C,s_i}^\gamma,v_{\mathcal C,s_i}^\gamma,\theta^*)$ ... introduce unlimited capacity and transit time $\gamma$ ...

\begin{algorithm}[h]
	\DontPrintSemicolon
	\caption{Integral Quickest Transshipments - Subroutine}
	\label{Alg:param_transit}
	\KwIn{a dynamic network $\N$ and a supply/demand vector $b$ with integral supplies, demands, and capacities, a time horizon  $\theta^*$, and a terminal/SOURCE?? $s_i$}
	\KwOut{a $\gamma$ s.t. $(\mathcal N_{\mathcal C,s_i}^\gamma,v_{\mathcal C,s_i}^\gamma,\theta^*)$ is feasible but $(\mathcal N_{\mathcal C,s_i}^{\gamma+\varepsilon},v_{\mathcal C,s_i}^{\gamma+\varepsilon},\theta^*)$ is infeasible}
	
	Set $l:=0$, $u:=\theta^*$\;
	\While{$(\mathcal N_{\mathcal C,s_i}^u,v_{\mathcal C,s_i}^u,\theta^*)$ is not tight}{
		Set $u':=\min_{u^*:d_{\mathcal C,s_i}^{u^*}=0}$ using (modified) Algorithm~\ref{alg_main}\;
		\uIf{$(\mathcal N_{\mathcal C,s_i}^{2u'-u},v_{\mathcal C,s_i}^{2u'-u},\theta^*)$ is feasible}
			{Set $l:= 2u'-u$ and then $u:=u'$}
		\Else {Set $u:= 2u'-u$}
		}
	\Return $u=l$
	
\end{algorithm}

\begin{lemma}
Algorithm~\ref{Alg:param_transit} terminates within $\tilde O(m\log m + k^2)$ iterations.
\end{lemma}



==> Figures/choice_of_j.tex <==
\begin{tikzpicture}
    %axis   
%axis 
    \draw[->, >=stealth', thick] (-0.5,0)  -- (10,0) node(xline)[below]
        {time $\theta$};
    \draw[->, >=stealth', thick] (0, -3) -- (0,2) node(yline)[right] {$d^\theta(X)$};

    \draw[thin, color = gray] (0,-1) -- (1,-1) -- (5,0.5)--(7,2);
    %
    \draw[thin, color = gray] (0,-2.2)--(2,-2.2)--(5,-1)--(8,2);

    \draw[thick, color = black] (0,-2.5) -- (1.5,-2.5)--(3,-2)--(4,-1)--(5,0)--(6,2) node[left, black] {$\scriptstyle S_i$} ;
    %
    \draw[thin, color=gray] (0,-2)--(2,-2)--(5,-1.5)--(7,-0.5)--(9,1.5)--(9.5,2);
    %
    \draw[thin, color=gray] (0,-1.5)--(1,-1.5)--(7,-1)--(8.5,0)--(10,1.5);
    
    \draw[thin, color=gray] (0,1)--(3,1.3)--(4,1.6)--(4.5,2);

    \draw[thin, color=gray] (0,0)--++(1,0.2)--++(0.5,0.5)--(1.7,2);

    \draw[thin, color=gray] (0,-1.25)--++(4.5,1)--++(3,1)--++(0.5,0.5)--(8.5,2);

    \draw[thick, color=black] (0,-0.5)--++(2,0.5)--++(2,0.8)--(5,2)node[black, left] {$\scriptstyle S_{i-1}$};

    %Iterations
    \draw[densely dashed, gray, name path = it1] (2,2) -- (2,-3);
    \node[below] at (2,0){$\theta_{i}$};


    \draw[densely dashed, gray, name path = it2] (5,2) -- (5,-3);
    \node[below] at (5,0){$\theta_{i}'$};

    %\node[below] at (7.5,0){$\theta_{i+2}$};
    \node[below] at (8.5,0){$\theta_{i+2}$};
    \draw[densely dashed, gray, name path = it2] (8,2) -- (8,-3);
    \draw[densely dashed, gray, name path = it2] (8.5,2) -- (8.5,-3);


    \coordinate (m1) at (2,-2.33333){};
    \coordinate (m2) at (5,-1.5){};
    \coordinate (m3) at (7.5,-0.666666){};

    \coordinate (m4) at (8.5,0){};

    \fill[red] (m1) circle (1.5pt);
    \fill[red] (m2) circle (1.5pt);
    \fill[red] (m4) circle (1.5pt);



    \coordinate (p1) at (3.2 ,-1.8);
    \coordinate (p2) at (5.8 ,-1.1);
    %lower envelope
    \draw[thick, color = red] (0,-2.5) -- (1.5,-2.5)--(3,-2)--(p1)--(5,-1.5)--(p2)--(7,-1)--(8.5,0)--(10,1.5);

    %Choice of j


    \fill[red] (8,-0.33333) circle (1.5pt);

    \begin{scope}
         %\fill (m2) rectangle (10,0.6);
          \clip(m2) rectangle (10,0.6);
          \draw[thick, color = purple, name path = j1] (m2) -- ++(2,2) ;
          \draw[thick, color = purple, name path = j2] (m2) -- ++(5,2.5);
          \draw[thick, color = purple, name path = j3] (m2) -- ++(8,2);
          \draw[thin, color = purple, dotted] (m2) -- ++(8,1);
          %\draw[very thick, color = purple, name path = j3] (m2) -- ++(6,2);
        %   \path [name intersections={of=xaxis and j2, by={j2_int}}];
        %   \path [name intersections={of=xaxis and j1, by={j1_int}}];
        %   \path [name intersections={of=xaxis and j3, by={j3_int}}];


        \fill[purple] (8,0) circle (1.5pt) node[black,above] {$\theta_{i+1}$};
        % \fill[purple] (j1_int) circle (1.5pt);
        % \fill[purple] (j3_int) circle (1.5pt);
    \end{scope}

    % \node at (4,-2.5) (a){slope $$};
    % \node at (3.9,-1) (b){};

    % \draw (a) edge[bend right = 25,-stealth] (b);


\end{tikzpicture}
